Unfolding Videos Dynamics via Taylor Expansion

Taking inspiration from physical motion, we present a new self-supervised dynamics learning strategy for videos: Video Time-Differentiation for Instance Discrimination (ViDiDi). ViDiDi is a simple and data-efficient strategy, readily applicable to existing self-supervised video representation learning frameworks based on instance discrimination. At its core, ViDiDi observes different aspects of a video through various orders of temporal derivatives of its frame sequence. These derivatives, along with the original frames, support the Taylor series expansion of the underlying continuous dynamics at discrete times, where higher-order derivatives emphasize higher-order motion features. ViDiDi learns a single neural network that encodes a video and its temporal derivatives into consistent embeddings following a balanced alternating learning algorithm. By learning consistent representations for original frames and derivatives, the encoder is steered to emphasize motion features over static backgrounds and uncover the hidden dynamics in original frames. Hence, video representations are better separated by dynamic features. We integrate ViDiDi into existing instance discrimination frameworks (VICReg, BYOL, and SimCLR) for pretraining on UCF101 or Kinetics and test on standard benchmarks including video retrieval, action recognition, and action detection. The performances are enhanced by a significant margin without the need for large models or extensive datasets.

==> sec/checklist.tex <==
\clearpage

\section*{NeurIPS Paper Checklist}

% %%% BEGIN INSTRUCTIONS %%%
% The checklist is designed to encourage best practices for responsible machine learning research, addressing issues of reproducibility, transparency, research ethics, and societal impact. Do not remove the checklist: {\bf The papers not including the checklist will be desk rejected.} The checklist should follow the references and follow the (optional) supplemental material.  The checklist does NOT count towards the page
% limit. 

% Please read the checklist guidelines carefully for information on how to answer these questions. For each question in the checklist:
% \begin{itemize}
%     \item You should answer \answerYes{}, \answerNo{}, or \answerNA{}.
%     \item \answerNA{} means either that the question is Not Applicable for that particular paper or the relevant information is Not Available.
%     \item Please provide a short (1–2 sentence) justification right after your answer (even for NA). 
%    % \item {\bf The papers not including the checklist will be desk rejected.}
% \end{itemize}

% {\bf The checklist answers are an integral part of your paper submission.} They are visible to the reviewers, area chairs, senior area chairs, and ethics reviewers. You will be asked to also include it (after eventual revisions) with the final version of your paper, and its final version will be published with the paper.

% The reviewers of your paper will be asked to use the checklist as one of the factors in their evaluation. While "\answerYes{}" is generally preferable to "\answerNo{}", it is perfectly acceptable to answer "\answerNo{}" provided a proper justification is given (e.g., "error bars are not reported because it would be too computationally expensive" or "we were unable to find the license for the dataset we used"). In general, answering "\answerNo{}" or "\answerNA{}" is not grounds for rejection. While the questions are phrased in a binary way, we acknowledge that the true answer is often more nuanced, so please just use your best judgment and write a justification to elaborate. All supporting evidence can appear either in the main paper or the supplemental material, provided in appendix. If you answer \answerYes{} to a question, in the justification please point to the section(s) where related material for the question can be found.

% IMPORTANT, please:
% \begin{itemize}
%     \item {\bf Delete this instruction block, but keep the section heading ``NeurIPS paper checklist"},
%     \item  {\bf Keep the checklist subsection headings, questions/answers and guidelines below.}
%     \item {\bf Do not modify the questions and only use the provided macros for your answers}.
% \end{itemize} 
 

%%% END INSTRUCTIONS %%%


\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The abstract introduced the paper's contributions and scope in proposing a new self-supervised video dynamics learning method presented in \Cref{sec:approach} and \Cref{sec:experiments}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A No or NA answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We provide discussions on limitations and future directions in \Cref{sec:discussion}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper has no limitation while the answer No means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate "Limitations" section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory Assumptions and Proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We do not propose theorems in the paper.  
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

    \item {\bf Experimental Result Reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We clearly explained the proposed methods and algorithms in \Cref{sec:approach}, as well as experiment setup in \Cref{sec:experiments} and \Cref{sec:detail}. The code will be released upon acceptance.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item If the paper includes experiments, a No answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and/or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerNo{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We haven't provided an open access code with detailed instructions upon submission, but will provide an open access code with detailed instructions upon acceptance.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so “No” is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental Setting/Details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer, etc.) necessary to understand the results?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We clearly explained the proposed methods and algorithms in \Cref{sec:approach}, as well as experiment setup in \Cref{sec:experiments} and \Cref{sec:detail}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment Statistical Significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We conduct main experiments for at least 3 times. We follow the standard train/val/test splits of the datasets.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The authors should answer "Yes" if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g. negative error rates).
        \item If error bars are reported in tables or plots, The authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments Compute Resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The required computing resources are justified in \Cref{sec:detail}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code Of Ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We follow the NeurIPS Code of Ethics.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer No, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader Impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We discuss the potential inspiration of the work to both machine vision and neuroscience.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that there is no societal impact of the work performed.
        \item If the authors answer NA or No, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pretrained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Our paper does not have such risks.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We properly cited and credited existing models and datasets.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New Assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We describe the proposed new frameworks and algorithms in details.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset/code/model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and Research with Human Subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We do not involve human subjects.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional Review Board (IRB) Approvals or Equivalent for Research with Human Subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We do not involve human subjects.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\end{enumerate}

==> sec/conclusion.tex <==
\vspace{-0.2cm}
\section{Conclusion}
\label{sec:discussion}
\vspace{-0.2cm}

In this paper, we introduce ViDiDi, a novel, data-efficient, and generalizable framework for self-supervised video representation. We utilize the Taylor series to unfold a video to multiple views through different orders of temporal derivatives and learn consistent representations among original clips and their derivatives following a balanced alternating learning strategy. ViDiDi learns to extract dynamic features instead of static shortcuts better, enhancing performance on common video representation learning tasks significantly.

Originating from our intuition of understanding the physical world, there are also parallels between this approach and human vision. The human eyes differentiate visual input into complementary retinal views with different spatial and temporal selectivity. The brain integrates these retinal views into holistic internal representations, allowing us to understand the world while being entirely unaware of the differential retinal views. This analogy provides an intriguing perspective on how machines and humans might align their mechanisms in visual processing and learning, which is not explored in the current scope of the paper. 

We identify multiple future directions as well. One is to represent different orders of dynamics through different sub-modules in the encoder. In this way, those encoders may teach one another and co-evolve during the learning process, learn different aspects of video dynamics, and be used for different purposes after training. Besides, we can apply Taylor expansion to other modalities or apply ViDiDi to other vision tasks that require more fine-grained understanding of video dynamics \cite{videosp} such as action segmentation \cite{Kuehne2014TheLO}. Moreover, due to computation limitations, we are unable to scale the model up to state-of-the-art video transformers using high-resolution inputs, which would be worth exploration for large-scale applications. Furthermore, a potentially fruitful direction is to use this approach to learn intuitive physics, supporting agents to understand, predict, and interact with the physical world, since the method's intuition also connects with understanding the physical world. 



==> sec/experiment.tex <==
\section{Experiments}
\label{sec:experiments}
\vspace{-0.1cm}
\subsection{Experiment Setup}
\vspace{-0.1cm}

% \textcolor{red}{Add some implementation details}

\noindent \textbf{Datasets.   }
We train and evaluate ViDiDi using human action video datasets. \textbf{UCF101} \cite{ucf101} includes 13k videos from $101$ classes. \textbf{HMDB51} \cite{hmdb51} contains 7k videos from $51$ classes. In addition, we also use larger and more diverse datasets, \textbf{K400} \cite{kinetics}, aka Kinetics400,  including 240k videos from $400$ classes, and \textbf{K200-40k}, including 40k videos from $200$ classes, as a subset of Kinetics $400$, helps verify data-efficiency. In our experiments, we pretrain models with UCF101, K400, or K200-40k and then test them with UCF101 or HMDB51, using split 1 for both datasets. \textbf{AVA} contains 280K videos from $60$ action classes, each video is annotated with spatiotemporal localization of human actions.

\noindent \textbf{Basics of networks and training.}
We use R3D-18 \cite{closer} as the default architecture for the video encoder. In addition, we also explore other architectures, namely R(2+1)D-18 \cite{closer}, MC3-18 \cite{closer}, and S3D \cite{s3d}. We test ViDiDi on instance discrimination methods including VICReg, SimCLR, and BYOL. During self-supervised pretraining, we remove the classification head and train the model up to the final global average pooling layer, followed by a MLP-based projection head. We pretrain the model for 400 epochs on UCF101 and K200-40k, and K400. The learning rate follows a cosine decay schedule \cite{sgdr} for all frameworks. A 10-epoch warmup is only employed for BYOL. Weight decay is  $1e-6$. We apply cosine-annealing of the momentum for BYOL as proposed in \cite{byol}. The temperature for SimCLR is $\alpha = 0.1$, and hyper-parameters for VICReg are $\lambda = 1.0, \mu = 1.0, \nu = 0.05$. We train all models with the LARS optimizer \cite{lars} utilizing a batch size of 64 on UCF101 and 256 on Kinetics, with learning rate $\eta = 1.2$. After pretraining, the projection head is discarded.

% \vspace{0.2cm}
\noindent \textbf{Downstream tasks.   } We follow the evaluation protocol in previous works \cite{cacl, coclr, cvrl}, including three types of downstream tasks. i) \textbf{\textit{Video retrieval.}} We encode videos with the pretrained encoder, sample videos in the testing set to query the top-k ($k=1,5,10$) closest videos in the training set. The retrieval is successful if at least one out of the $k$ retrieved training videos is from the same class as the query video. ii) \textbf{\textit{Action recognition.}} We add a linear classification head to the pretrained model, and fine-tune this model end-to-end for 100 epoch for action classification. We report the top-1 accuracy. iii) \textbf{\textit{Action detection}.} We follow \cite{cvrl} to finetune the pretrained model as a detector within a Faster R-CNN  pipeline on AVA for 20 epochs, and report mean Average Precision (mAP). More details are in \cref{sec:detail} for both pertaining and testing.

\vspace{-0.1cm}
\subsection{Comparisons with Previous Works}
\vspace{-0.1cm}

Results on both video retrieval (\cref{tab:nnv}) and action recognition (\cref{tab:tune}) suggest that ViDiDi outperforms prior models. Compared to other models trained on Kinetics, ViDiDi-VIC achieves the highest accuracy using K400, while also reaching compatible performance using UCF101 or K200-40k subset for pretraining. Besides, ViDiDi-BYOL achieves the best performance in action recognition on HMDB51, by a significant margin of $5.1$\% over the recent TCLR method \cite{tclr}. Importantly, ViDiDi supports efficient use of data. Its performance gain is most significant in the scenario of training with smaller datasets. We discuss this with more details in the following section.

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[t]
\scriptsize
% \setlength{\tabcolsep}{4pt}
% \footnotesize
\centering
\caption{\textbf{ViDiDi surpasses previous works on action recognition after finetuning.}}
\begin{tabular}{@{}cccccc@{}}
\toprule
Method             & Net            & Input    & Pretrained & UCF        & HMDB        \\ \midrule
VCOP \cite{vcop}              & R3D-18     & 16 × 112 & UCF101     & 64.9          & 29.5          \\
VCP \cite{vcp}              & R3D-18     & 16 × 112 & UCF101     & 66.0          & 31.5          \\
3D-RotNet \cite{3drotnet}         & R3D-18         & 16 × 112 & K600       & 66.0          & 37.1          \\
DPC \cite{dpc}               & R3D-18         & 25 × 128 & K400       & 68.2          & 34.5          \\
VideoMoCo \cite{videomoco}         & R3D-18         & 32 × 112 & K400       & 74.1          & 43.6          \\
RTT \cite{rtt}               & R3D-18         & 16 × 112 & K600       & 79.3          & 49.8          \\
VIE \cite{vie}            & R3D-18         & 16 × 112 & K400       & 72.3          & 44.8          \\
RSPNet \cite{rspnet}            & R3D-18         & 16 × 112 & K400       & 74.3          & 41.8          \\
VTHCL \cite{vthcl}            & R3D-18         & 8 × 224 & K400       & 80.6          & 48.6          \\
CPNet \cite{cpnet}              & R3D-18     & 16 × 112 & K400       & 80.8          & 52.8          \\
CPNet \cite{cpnet}             & R3D-18     & 16 × 112 & UCF101       & 77.2          & 46.3          \\
CACL \cite{cacl}              & T+C3D     & 16 × 112 & K400       & 77.5          & -          \\
CACL \cite{cacl}             & T+R3D     & 16 × 112 & UCF101       & 77.5          & 43.8          \\
% TCLR \cite{tclr}              & C3D     & 16 × 112 & UCF101       & 76.1          & 48.6          \\
TCLR \cite{tclr}              & R3D-18     & 16 × 112 & UCF101       & 82.4          & 52.9          \\
% \textbf{ViDiDi-SimCLR}  & R3D-18   & 16 × 112    & UCF101     & \textbf{80.6}   & \textbf{51.0}   \\
\textbf{ViDiDi-BYOL} & R3D-18         & 16 × 112 & UCF101     & \textbf{83.4} & \textbf{58.0} \\
\textbf{ViDiDi-VIC} & R3D-18         & 16 × 112 & UCF101     & \textbf{82.3} & \textbf{53.4} \\
\textbf{ViDiDi-VIC} & R3D-18         & 16 × 112 & K200-40k   & \textbf{82.7}             & \textbf{54.2} \\
\textbf{ViDiDi-VIC} & R3D-18         & 16 × 112 & K400   & \textbf{83.2}             & \textbf{55.8} \\ \midrule
VCOP \cite{vcop}              & R(2+1)D-18     & 16 × 112 & UCF101     & 72.4          & 30.9          \\
VCP \cite{vcp}              & R(2+1)D-18     & 16 × 112 & UCF101     & 66.3          & 32.2          \\
PacePred \cite{pacepred}          & R(2+1)D-18     & 16 × 112 & K400       & 77.1          & 36.6          \\
VideoMoCo \cite{videomoco}        & R(2+1)D-18     & 32 × 112 & K400       & 78.7          & 49.2          \\
V3S \cite{v3s}               & R(2+1)D-18     & 16 × 112 & K400       & 79.2          & 40.4          \\
RSPNet \cite{rspnet}            & R(2+1)D-18     & 16 × 112 & K400       & 81.1          & 44.6          \\
RTT \cite{rtt}               & R(2+1)D-18     & 16 × 112 & UCF101     & 81.6          & 46.4          \\
CPNet \cite{cpnet}               & R(2+1)D-18     & 16 × 112 & UCF101     & 81.8          & 51.2          \\
CACL \cite{cacl}              & T+R(2+1)D & 16 × 112 & UCF101     & 82.5          & 48.8          \\
\textbf{ViDiDi-VIC} & R(2+1)D-18     & 16 × 112 & UCF101     & \textbf{83.0} & \textbf{54.9} \\ \bottomrule
\end{tabular}
\label{tab:tune}
\end{table}

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[t]
% \small
% \setlength{\tabcolsep}{4pt}
\scriptsize
% \setlength{\tabcolsep}{3pt}
% \footnotesize
\centering
\caption{\textbf{ViDiDi surpasses previous SSL models on video retrieval.} T + C3D means training with an additional transformer.}
\begin{tabular}{@{}ccccccccc@{}}
\toprule
\multirow{2}{*}{Method} & \multirow{2}{*}{Net} & \multirow{2}{*}{Pretrained} & \multicolumn{3}{c}{UCF101}                                                     & \multicolumn{3}{c}{HMDB51}                                                    \\ \cmidrule(l){4-9} 
                        &                      &                             & 1                        & 5                        & 10                       & 1                       & 5                        & 10                       \\ \midrule
SpeedNet \cite{speednet}                & S3D-G                & K400                        & 13.0                     & 28.1                     & 37.5                     & -                       & -                        & -                        \\
RTT \cite{rtt}                    & R3D-18               & K600                        & 26.1                     & 48.5                     & 59.1                     & -                       & -                        & -                        \\
RSPNet \cite{rspnet}                  & R3D-18               & K400                        & 41.1                     & 59.4                     & 68.4                     & -                       & -                        & -                        \\
CoCLR \cite{coclr}                  & S3D                  & K400                        & 46.3                     & 62.8                     & 69.5                     & 20.6                    & 43.0                     & 54.0                     \\
CACL \cite{cacl}                   & T+C3D           & K400                        & 44.2                     & 63.1                     & 71.9                     & -                       & -                        & -                        \\
\textbf{ViDiDi-VIC}      & R3D-18               & K200-40k                    & \textbf{49.5}            & \textbf{63.4}            & \textbf{71.0}            & \textbf{24.7}           & \textbf{45.4}            & \textbf{56.0}            \\
\textbf{ViDiDi-VIC}      & R3D-18               & K400                    & \textbf{51.2}            & \textbf{64.6}            & \textbf{72.6}            & \textbf{25.0}           & \textbf{47.2}            & \textbf{60.9}            \\
% \textbf{ViDiDi*-VIC}     & R3D-18               & K200-40k                    & \textbf{50.6}            & \textbf{64.8}            & \textbf{73.0}            & \textbf{24.6}           & \textbf{47.0}            & \textbf{60.7}            \\ 
\midrule
VCOP \cite{vcop}                  & R3D-18               & UCF101                      & 14.1                     & 30.3                     & 40.0                     & 7.6                     & 22.9                     & 34.4                     \\
VCP \cite{vcp}                    & R3D-18               & UCF101                      & 18.6 & 33.6 & 42.5 & 7.6 & 24.4 & 33.6 \\
PacePred \cite{pacepred}               & R3D-18               & UCF101                      & 23.8                     & 38.1                     & 46.4                     & 9.6                     & 26.9                     & 41.1                     \\
PRP \cite{prp}                    & R3D-18               & UCF101                      & 22.8                     & 38.5                     & 46.7                     & 8.2                     & 25.8                     & 38.5                     \\
V3S \cite{v3s}                    & R3D-18               & UCF101                      & 28.3                     & 43.7                     & 51.3                     & 10.8                    & 30.6                     & 42.3                     \\
CACL \cite{cacl}                   & T+R3D           & UCF101                      & 41.1                     & 59.2                     & 67.3                     & 17.6                    & 36.7                     & 48.4                     \\
% TransRank-ST            & R3D-18               & UCF101                      & 46.5                     & 63.7                     & 72.8                     & 19.4                    & 45.4                     & 59.1                     \\
\textbf{ViDiDi-VIC}      & R3D-18               & UCF101                      & \textbf{47.6}            & \textbf{60.9}            & \textbf{68.6 }           & \textbf{19.7}           & \textbf{40.5}            & \textbf{55.1}            \\
% \textbf{ViDiDi*-VIC}     & R3D-18               & UCF101                      & \textbf{49.2}            & \textbf{64.7}            & \textbf{73.1}            & \textbf{20.2}           & \textbf{45.6}            & \textbf{59.4}            \\ 
\bottomrule
\end{tabular}
\label{tab:nnv}
\end{table}


% \begin{figure}[t]
%   \centering
%    \includegraphics[width=\linewidth]{figure/perform_2d2.pdf}
%    \caption{\textbf{Data efficiency and accuracy compared with previous works.} ViDiDi boosts action recognition accuracy on UCF101 and HMDB51 after fine-tuning.}
%    \label{fig:sota}
%    \vspace{-0.5cm}
% \end{figure}



\subsection{Data-efficiency and Generalizability}
\label{sec:efficiency}

% \textcolor{red}{Discuss data-efficiency in detail}

\noindent \textbf{Efficient learning with limited data.   }
ViDiDi learns effective video representations with limited data. As presented in \cref{tab:nnv} and \cref{tab:tune}, pretrained on small dataset UCF101 or K200-40k, ViDiDi surpasses prior video representation learning works pretrained on large-scale K400 or K600 dataset. Further, ViDiDi-VIC pretrained on UCF101 or K200-40k outperforms its baseline method VICReg pretrained on K400, and also reaches compatible performance as ViDiDi-VIC pretrained on K400, as shown in \cref{tab:nnv_general}. This aligns with our intuition that holistic learning of derivatives and original frames can steer the encoder to uncover dynamics features as our intuition discussed in \cref{sec:taylor}. Such a strategy efficiently uncovers dynamic features with limited data and does not rely on a more diverse dataset. To gain insights into how ViDiDi works, we further visualize the spatio-temporal attention in \cref{sec:visualize} , and find that ViDiDi attends to dynamic parts in original frames but VICReg  attends to background shortcuts. 


\begin{table}[t]
\scriptsize
% \setlength{\tabcolsep}{4pt}
% \footnotesize
\centering
\caption{\textbf{Video Retrieval. ViDiDi exhibits efficient learning and generalizes across different methods.}}
\begin{tabular}{@{}cccccccc@{}}
\toprule
\multirow{2}{*}{Method} & \multirow{2}{*}{Pretrained} & \multicolumn{3}{c}{UCF101} & \multicolumn{3}{c}{HMDB51} \\ \cmidrule(l){3-8} 
                        &                             & 1       & 5       & 10     & 1       & 5       & 10     \\ \midrule
SimCLR                  & UCF101                      & 29.6    & 41.4    & 49.3   & 17.5    & 34.7    & 45.1   \\
\textbf{ViDiDi-SimCLR}            & UCF101                      & \textbf{38.3}    & \textbf{54.6}    & \textbf{64.5}   & \textbf{17.5}    & \textbf{38.9}    & \textbf{52.4}   \\
\midrule
BYOL                    & UCF101                      & 32.2    & 43.0    & 50.5   & 13.8    & 31.1    & 44.4   \\
\textbf{ViDiDi-BYOL}              & UCF101                      & \textbf{43.7}    & \textbf{60.4}    & \textbf{70.1}   & \textbf{19.3}    & \textbf{44.1}    & \textbf{56.6}   \\
\midrule
VICReg                  & UCF101                      & 31.1    & 43.6    & 50.9   & 15.7    & 33.7    & 44.5   \\
\textbf{ViDiDi-VIC}               & UCF101                      & \textbf{47.6}    & \textbf{60.9}    & \textbf{68.6}   & \textbf{19.7}    & \textbf{40.5}    & \textbf{55.1}   \\
\midrule
% VICReg                  & K200-40k                    & 38.8    & 50.7    & 58.7   & 20.0    & 39.6    & 50.9   \\
VICReg                & K400                    & 41.9    & 56.5    & 64.8   & 21.7    & 44.1    & 56.1   \\
% VICReg                  & K200-80k                    & 40.9    & 54.5    & 62.4   & 20.5    & 44.2    & 54.8   \\ 
\textbf{ViDiDi-VIC}               & K400                    & \textbf{51.2}    & \textbf{64.6}    & \textbf{72.6}   & \textbf{25.0}   & \textbf{47.2}   &  \textbf{60.9}  \\
\textbf{ViDiDi-VIC}               & K200-40k                    & \textbf{49.5}    & \textbf{63.4}    & \textbf{71.0}   & \textbf{24.7}    & \textbf{45.4}    & \textbf{56.0}   \\
% ViDiDi*-VIC              & UCF101                      & 49.2    & 64.7    & 73.1   & 20.2    & 45.1    & 59.4   \\
% ViDiDi*-VIC             & K200-40k                    & 50.6    & 64.8    & 73.0   & 24.6    & 47.0    & 60.7   \\ 
\bottomrule
\end{tabular}
\label{tab:nnv_general}
\end{table}

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[t]
\scriptsize
\centering
\caption{\textbf{Action Detection. ViDiDi exhibits better spatiotemporal action localization.}}
\begin{tabular}{@{}cccllll@{}}
\toprule
Method & VICReg & \textbf{ViDiDi-VIC} & SimCLR & \textbf{ViDiDi-SimCLR} & BYOL  & \textbf{ViDiDi-BYOL} \\ \midrule
mAP    & 0.089  & \textbf{0.106}      & 0.079  & \textbf{0.094}         & 0.087 & \textbf{0.118}       \\ \bottomrule
\end{tabular}
\label{tab:ava}
\vspace{-0.3cm}
\end{table}

\noindent \textbf{Generalization across methods, backbones, and downstream tasks.   }
ViDiDi is compatible with multiple existing frameworks based on instance discrimination. We combine ViDiDi with SimCLR, BYOL, and VICReg and find that ViDiDi improves the performance of video retrieval for each of these frameworks. As shown in \cref{tab:nnv_general}, the performance gain is remarkable (up to 16.5\%) and consistent across the three frameworks on video retrieval. With fine-tuning, ViDiDi significantly improves the performance (up to 18.0\%) over their counterparts without ViDiDi on action recognition, as shown in \cref{fig:generalization}. Further, when finetuned on action detection, ViDiDi also exhibits consistent performance gain as illustrated in \cref{tab:ava}. ViDiDi is also applicable to different encoder architectures, including R3D-18, R(2+1)D-18, MC3-18, and S3D. As shown in \cref{tab:tune_general_net}, the performance gain in video retrieval is significant for every encoder architecture tested herein, ranging from 13.7\% to 17.0\% in terms of top-1 accuracy. 


% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[t]
\scriptsize
% \setlength{\tabcolsep}{4pt}
% \footnotesize
\centering
\caption{\textbf{Video Retrieval. ViDiDi generalizes to other backbones.}}
\begin{tabular}{@{}cccccccc@{}}
\toprule
\multirow{2}{*}{Net}        & \multirow{2}{*}{Method} & \multicolumn{3}{c}{UCF101} & \multicolumn{3}{c}{HMDB51} \\ \cmidrule(l){3-8} 
                            &                         & 1       & 5       & 10     & 1       & 5       & 10     \\ \midrule
% \multirow{2}{*}{R3D-18}     & VICReg                  & 31.1    & 43.6    & 50.9   & 15.7    & 33.7    & 44.5   \\
%                             & \textbf{ViDiDi-VIC}                & \textbf{47.6}    & \textbf{60.9}    & \textbf{68.6}   & \textbf{19.7}    & \textbf{40.5}    & \textbf{55.1}   \\ \midrule
\multirow{2}{*}{R(2+1)D-18} & VICReg                  & 30.2    & 44.1    & 51.4   & 15.8    & 33.6    & 45.5   \\
                            & \textbf{ViDiDi-VIC}                & \textbf{47.2}    & \textbf{62.6}    & \textbf{69.8}   & \textbf{20.6}    & \textbf{44.1}    & \textbf{57.7}  \\ \midrule
\multirow{2}{*}{MC3-18}     & VICReg                  & 31.9    & 44.4    & 51.4   & 15.6    & 35.6    & 46.1   \\
                            & \textbf{ViDiDi-VIC}                & \textbf{44.1}    & \textbf{59.8}    & \textbf{68.0}   & \textbf{20.3}    & \textbf{40.3}    & \textbf{53.4}   \\ \midrule
\multirow{2}{*}{S3D}        & VICReg                  & 29.2    & 41.9    & 49.2   & 12.8    & 29.8    & 40.9   \\
                            & \textbf{ViDiDi-VIC}                & \textbf{42.9}    & \textbf{59.0}    & \textbf{67.5}   & \textbf{18.4}    & \textbf{38.4}    & \textbf{51.4}   \\ \bottomrule
\end{tabular}
\label{tab:tune_general_net}
\end{table}
\vspace{-0.2cm}
\subsection{Visualization}
\label{sec:visualize}
\vspace{-0.2cm}

\begin{figure}[ht]
  \centering
   \includegraphics[width=\linewidth]{figure/sil_plot2.pdf}
   \caption{\textbf{Silhouette scores and t-SNE of top 5 classes} from VICReg (left) and ViDiDi-VIC (right).}
   \label{fig:score_tsne}
   \vspace{-0.2cm}
\end{figure}

% \vspace{-0.5cm}
% \vspace{-0.1cm}
\noindent \textbf{Clustering in the latent space.   } We also examine how video representations from different action classes are distributed in the latent space. We use t-SNE \cite{tsne} to visualize the representations from five classes. As shown in \cref{fig:score_tsne}, video representations learned with ViDiDi are better clustered by action classes), showing further separation across distinct classes. Beyond visual inspection, the Silhouette score \cite{sscore} in \cref{tab:score} in appendix and \cref{fig:score_tsne} quantifies the degree of separation and shows better segregation by video classes with ViDiDi. 



\vspace{-0.1cm}
\noindent \textbf{Spatio-temporal attention.   } To better understand the model's behavior, we visualize the spatiotemporal attention using Saliency Tubes \cite{SaliencyTV}. ViDiDi leads the model to attend to dynamic aspects of the video, such as motions and interactions, rather than static backgrounds as shown in \cref{fig:attention}. The model's attention to dynamics is generalizable to videos that the model has not seen.  These results align with our intuition that ViDiDi attends to dynamic parts and avoids learning static content as a learning shortcut, resulting in efficient utilization of data as discussed in \cref{sec:efficiency}. 

\begin{figure}[t]
\centering
\begin{subfigure}[t]{0.325\linewidth}
\centering
   \caption*{\textbf{Frames}}
\end{subfigure}%
    \hspace{.0005\linewidth}
\begin{subfigure}[t]{0.325\linewidth}
\centering
\caption*{\textbf{Attn of VIC}}
\end{subfigure}%
    \hspace{.0005\linewidth}
\begin{subfigure}[t]{0.325\linewidth}
\centering
\caption*{\textbf{Attn of ViDiDi-VIC}}
\end{subfigure}
   \begin{subfigure}[t]{\linewidth}
    \includegraphics[width=0.1\linewidth]{figure/CuttingInKitchen/img_000.png}
    \includegraphics[width=0.1\linewidth]{figure/CuttingInKitchen/img_005.png}
    \includegraphics[width=0.1\linewidth]{figure/CuttingInKitchen/img_010.png}
    \hspace{.0005\linewidth}
    \includegraphics[width=0.1\linewidth]{figure/CuttingInKitchen/heatmap_000.png}
    \includegraphics[width=0.1\linewidth]{figure/CuttingInKitchen/heatmap_005.png}
    \includegraphics[width=0.1\linewidth]{figure/CuttingInKitchen/heatmap_010.png}
    \hspace{.0005\linewidth}
    \includegraphics[width=0.1\linewidth]{figure/CuttingInKitchen/didi/heatmap_000.png}
    \includegraphics[width=0.1\linewidth]{figure/CuttingInKitchen/didi/heatmap_005.png}
    \includegraphics[width=0.1\linewidth]{figure/CuttingInKitchen/didi/heatmap_010.png}
    % \caption{Cutting In Kitchen}
\end{subfigure}

\vspace{.02\linewidth}
\begin{subfigure}[t]{\linewidth}
    \includegraphics[width=0.1\linewidth]{figure/PlayingCello/img_000.png}
    \includegraphics[width=0.1\linewidth]{figure/PlayingCello/img_005.png}
    \includegraphics[width=0.1\linewidth]{figure/PlayingCello/img_010.png}
    \hspace{.0005\linewidth}
    \includegraphics[width=0.1\linewidth]{figure/PlayingCello/heatmap_000.png}
    \includegraphics[width=0.1\linewidth]{figure/PlayingCello/heatmap_005.png}
    \includegraphics[width=0.1\linewidth]{figure/PlayingCello/heatmap_010.png}
    \hspace{.0005\linewidth}
    \includegraphics[width=0.1\linewidth]{figure/PlayingCello/didi/heatmap_000.png}
    \includegraphics[width=0.1\linewidth]{figure/PlayingCello/didi/heatmap_005.png}
    \includegraphics[width=0.1\linewidth]{figure/PlayingCello/didi/heatmap_010.png}
    % \caption{Playing Cello}
\end{subfigure}

\vspace{.02\linewidth}
\begin{subfigure}[t]{\linewidth}
    \includegraphics[width=0.1\linewidth]{figure/ApplyLipstick/img_000.png}
    \includegraphics[width=0.1\linewidth]{figure/ApplyLipstick/img_005.png}
    \includegraphics[width=0.1\linewidth]{figure/ApplyLipstick/img_010.png}
    \hspace{.0005\linewidth}
    \includegraphics[width=0.1\linewidth]{figure/ApplyLipstick/heatmap_000.png}
    \includegraphics[width=0.1\linewidth]{figure/ApplyLipstick/heatmap_005.png}
    \includegraphics[width=0.1\linewidth]{figure/ApplyLipstick/heatmap_010.png}
    \hspace{.0005\linewidth}
    \includegraphics[width=0.1\linewidth]{figure/ApplyLipstick/didi/heatmap_000.png}
    \includegraphics[width=0.1\linewidth]{figure/ApplyLipstick/didi/heatmap_005.png}
    \includegraphics[width=0.1\linewidth]{figure/ApplyLipstick/didi/heatmap_010.png}
    % \caption{Apply Lip stick}
\end{subfigure}

% \vspace{.02\linewidth}
% \begin{subfigure}[t]{\linewidth}
%     \includegraphics[width=0.1\linewidth]{figure/Biking/img_064.png}
%     \includegraphics[width=0.1\linewidth]{figure/Biking/img_069.png}
%     \includegraphics[width=0.1\linewidth]{figure/Biking/img_074.png}
%     \hspace{.0005\linewidth}
%     \includegraphics[width=0.1\linewidth]{figure/Biking/heatmap_048.png}
%     \includegraphics[width=0.1\linewidth]{figure/Biking/heatmap_053.png}
%     \includegraphics[width=0.1\linewidth]{figure/Biking/heatmap_058.png}
%     \hspace{.0005\linewidth}
%     \includegraphics[width=0.1\linewidth]{figure/Biking/didi/heatmap_048.png}
%     \includegraphics[width=0.1\linewidth]{figure/Biking/didi/heatmap_053.png}
%     \includegraphics[width=0.1\linewidth]{figure/Biking/didi/heatmap_058.png}
%     % \caption{Biking}
% \end{subfigure}

\vspace{.02\linewidth}
\begin{subfigure}[t]{\linewidth}
    \includegraphics[width=0.1\linewidth]{figure/HorseRiding/img_160.png}
    \includegraphics[width=0.1\linewidth]{figure/HorseRiding/img_176.png}
    \includegraphics[width=0.1\linewidth]{figure/HorseRiding/img_215.png}
    \hspace{.0005\linewidth}
    \includegraphics[width=0.1\linewidth]{figure/HorseRiding/heatmap_140.png}
    \includegraphics[width=0.1\linewidth]{figure/HorseRiding/heatmap_155.png}
    \includegraphics[width=0.1\linewidth]{figure/HorseRiding/heatmap_195.png}
    \hspace{.0005\linewidth}
    \includegraphics[width=0.1\linewidth]{figure/HorseRiding/didi/heatmap_141.png}
    \includegraphics[width=0.1\linewidth]{figure/HorseRiding/didi/heatmap_155.png}
    \includegraphics[width=0.1\linewidth]{figure/HorseRiding/didi/heatmap_193.png}
    % \caption{Horse Riding}
\end{subfigure}

\vspace{.02\linewidth}
\begin{subfigure}[t]{\linewidth}
    \includegraphics[width=0.1\linewidth]{figure/bike/img_070.png}
    \includegraphics[width=0.1\linewidth]{figure/bike/img_090.png}
    \includegraphics[width=0.1\linewidth]{figure/bike/img_110.png}
    \hspace{.0005\linewidth}
    \includegraphics[width=0.1\linewidth]{figure/bike/heatmap_050.png}
    \includegraphics[width=0.1\linewidth]{figure/bike/heatmap_070.png}
    \includegraphics[width=0.1\linewidth]{figure/bike/heatmap_090.png}
    \hspace{.0005\linewidth}
    \includegraphics[width=0.1\linewidth]{figure/bike/didi/heatmap_050.png}
    \includegraphics[width=0.1\linewidth]{figure/bike/didi/heatmap_070.png}
    \includegraphics[width=0.1\linewidth]{figure/bike/didi/heatmap_090.png}
    % \caption{Playing Cello}
\end{subfigure}
   \caption{\textbf{Spatiotemporal attention on UCF and HMDB51.} Left: Original frames. Middle: Attention from VIC. Right: Attention from ViDiDi-VIC.}
   \label{fig:attention}
   \label{fig:attention_hmdb}
   \vspace{-0.3cm}
\end{figure}


\section{Ablation Study}
\label{sec:ablation}

ViDiDi involves multiple methodological choices, including 1) the order of derivatives, 2) how to pair different orders of derivatives as the input to two-stream video encoders, and 3) how to prescribe the learning schedule over different pairings. We perform ablation studies to test each design choice.  

For the order of derivatives, we consider up to the $2^{nd}$ derivative. For pairing, we consider pairing derivatives in the same order ($1^{st}$ vs. $1^{st}$, $2^{nd}$ vs. $2^{nd}$, etc.) or between different orders ($1^{st}$ vs. $0^{th}$, $1^{st}$ vs. $2^{nd}$, etc.), respectively. For scheduling, we consider either random vs. scheduled selection of input pairs. With random selection, temporal differentiation is essentially treated as additional data augmentation. In contrast, the scheduled selection (\cref{alg:schedule}) aims to provide a balanced and structured way for the model to learn from various orders of temporal derivatives, where higher order derivatives are intuitively used as guidance of learning the original frames.

As shown in \cref{tab:ablation}, results demonstrate a progressive improvement in the model's performance in video retrieval, given a higher order of derivatives (from the $1^{st}$ to $2^{nd}$ order), given mixed pairing, and given scheduled selection of input pairs. Therefore, temporal differentiation is not merely another data augmentation trick. Invariance to different orders of temporal derivatives is a valuable principle for SSL of video representations that lead to better performance in downstream tasks. To leverage this principle, it is beneficial to design mixed pairing and prescribe a learning schedule that provides a balanced and holistic view of different orders of temporal dynamics inherent to videos. Details about how we design the groups of models in \cref{tab:ablation} are summarized below:
\begin{itemize}
    \item \textbf{Base}: The direct extension of VICReg. 
    \item \textbf{+Random $1^{st}$}: Add $1^{st}$ order derivatives as random augmentation. 
    \item \textbf{+Random $1^{st}$ \& $2^{nd}$}: Add $1^{st}$ and $2^{nd}$ order derivatives as random augmentation. 
    \item \textbf{Reverse ViDiDi-VIC}: Reverse the order of pair alternation by epoch in ViDiDi, i.e., line 1-9 in \cref{alg:schedule}.
    \item \textbf{+Schedule $1^{st}$}: Alternate pairs across epochs in the order $(\frac{\partial \bm V}{\partial t}, \frac{\partial \bm V'}{\partial t}) \rightarrow (\bm V, \bm V') \rightarrow (\frac{\partial \bm V}{\partial t}, \frac{\partial \bm V'}{\partial t}) \rightarrow \dots$. 
    \item \textbf{+Schedule $1^{st}$ \& Mix}: switch pairs by epoch in the order $(\frac{\partial \bm V}{\partial t}, \frac{\partial \bm V'}{\partial t}) \rightarrow (\frac{\partial \bm V}{\partial t}, \bm V') \rightarrow (\bm V, \bm V') \rightarrow (\frac{\partial \bm V}{\partial t}, \frac{\partial \bm V'}{\partial t}) \rightarrow \dots$.
    \item \textbf{+Schedule $1^{st}$ \& $2^{nd}$} and \textbf{+Schedule $1^{st}$ \& $2^{nd}$ \& Mix}: Build upon +Schedule $1^{st}$ and +Schedule $1^{st}$ \& Mix accordingly with random differentiation at each batch to utilize $2^{nd}$ order derivatives.
\end{itemize}


\begin{table}[ht]
\scriptsize
% \setlength{\tabcolsep}{16pt}
% \footnotesize
\centering
\caption{\textbf{Ablation Study.} Video retrieval performance on UCF101 with different design choices.}
\begin{tabular}{@{}lccc@{}}
\toprule
\multirow{2}{*}{Method}                  & \multicolumn{3}{c}{UCF101}                    \\ \cmidrule(l){2-4} 
                                         & 1             & 5             & 10            \\ \midrule
Base (VICReg)                            & 31.1          & 43.6          & 50.9          \\
\midrule
+Random $1^{st}$                              & 35.2          & 47.7          & 56.1          \\
+Random $1^{st}$ \& $2^{nd}$             & 36.2          & 48.6          & 55.8          \\
Reverse ViDiDi-VIC & 39.1 & 54.7 & 62.9 \\
\midrule
+Schedule $1^{st}$                            & 37.1          & 50.3          & 58.2          \\
+Schedule $1^{st}$ \& Mix                     & 39.3          & 53.2          & 60.9          \\
\midrule
+Schedule $1^{st}$ \& $2^{nd}$                     & 40.7          & 56.5          & 64.0          \\
+Schedule $1^{st}$ \& $2^{nd}$ \& Mix              & 43.0          & 59.2          & 66.6          \\
\midrule
ViDiDi-VIC & \textbf{47.6} & \textbf{60.9} & \textbf{68.6} \\ \bottomrule
\end{tabular}
\label{tab:ablation}
\end{table}



==> sec/intro.tex <==
\section{Introduction}
\label{sec:intro}

% \syc{Shrink}


Learning video representations is central to various aspects of video understanding, such as action recognition \cite{ucf101, hmdb51}, video retrieval \cite{cacl, wang2021negative}, and action detection \cite{Gu2017AVAAV}. While supervised learning requires expensive video labeling \cite{kinetics}, recent works highlight the strengths of self-supervised learning (SSL) from unlabeled videos \cite{coclr, cvrl, tclr} with a large number of training videos. 
% but tend to demand a very large amount of training videos and thus computationally expensive. 
% Gaining inspiration from intuitive understanding of physical motion, we propose an intuitive and data efficienct learning method to unfold dynamics using the Taylor expansion. 

\begin{figure}[ht]
  \centering
    \begin{subfigure}[b]{0.48\textwidth}
         \centering
         \includegraphics[width=\linewidth]{figure/graph_illus2.pdf}
         \caption{}
         \label{fig:onecol}
     \end{subfigure}
     \hfill
    \begin{subfigure}[b]{0.48\textwidth}
         \centering
         \includegraphics[width=\linewidth]{figure/bar_plot.pdf}
         \caption{}
         \label{fig:generalization}
     \end{subfigure}
   \caption{\textbf{Method Overview}. (a) The ViDiDi method evaluates temporal derivatives of video clips through Taylor expansion, uses the same encoder to embed them into the latent space, and converges their representations for the same video while diverging those from different videos. (b) Pretraining via ViDiDi enhances existing instance discrimination methods significantly on action recognition.}
\end{figure}

One popular strategy for SSL on video representations uses instance discrimination objectives, such as SimCLR \cite{simclr}, initially demonstrated for images \cite{byol, simclr, moco, vicreg, swav} and then generalized to videos \cite{videomoco, rbyol, cvrl}. In images, models learn to pair together latent representations for the same instance under different augmented views. Such models effectively filter out lower-level details and generate abstract representations useful for higher-level tasks. When adapting this approach to videos, previous methods often use clips from different times as separate views of the same video, treating time as an additional spatial dimension. However, learning consistent representations across clips may cause models to prioritize static content (e.g., background scenes) over dynamic features (e.g., motion, action, and interaction), which are often essential to video understanding \cite{ucf101, hmdb51, kinetics, randomwalk, VideoHiGraph, RTDNet, bmn}. Despite some pretext tasks handling time in distinction from space \cite{videomoco, rbyol, cvrl, cacl, vthcl, coclr, tequi}, they are not generalizable or principled. In contrast, we utilize the unique role of time in "unfolding" continuous real-world dynamics.


In this paper, we introduce a generalizable and data-efficient method for improved dynamics learning, applicable to self-supervised video representation learning through instance discrimination. Central to our approach, we view a video not just as a sequence of discrete frames but as a continuous and dynamic process. We use the Taylor series expansion to express this continuous process as a weighted sum of its temporal derivatives at each frame. Using the physical motion as a metaphor, the zeroth-order derivative represents each frame itself, analogous to position. The first-order derivative captures the immediate motion between frames, analogous to velocity. The second-order derivative reveals the rate of change in this motion, analogous to acceleration. We train models to align representations for the original video and its first and second-order temporal derivatives, such that the learned representations encode the underlying dynamics more consistently among different orders of temporal differentiation (\cref{fig:onecol}). This method mirrors our intuitive perception of motion in the physical world, where a holistic understanding of position, velocity, and acceleration altogether helps us relate an object's trajectory to the underlying laws of physics. 

Herein, we refer to this approach as Video Time-Differentiation for Instance Discrimination (ViDiDi). We have implemented ViDiDi across three SSL methods using instance discrimination, including VICReg \cite{vicreg}, BYOL \cite{byol}, and SimCLR \cite{simclr}. ViDiDi is not merely an image-processing approach. It introduces new perspectives on understanding dynamic data including but not limited to videos, and uses a balanced alternating learning strategy to guide the learning process. We tested ViDiDi with different encoder architectures as well as different learning objectives. Pretrained on UCF101 or Kinetics, our method demonstrates excellent generalizability and data efficacy on standard benchmarks including action recognition (\cref{fig:generalization}) and video retrieval. 

% \qq{The highlight of the contribution is quite important. I feel there are too many bullet points, we should merge to three points at most. I feel 2 and 3 can be combined, and 4 and 5. Additionally, I would change novel to new, or something modest. }

Our contributions are summarized as follows: 
\begin{itemize}[leftmargin=*]
    \item Introducing \textit{a new view} for representing \textit{continuous dynamics} with different orders of temporal derivatives using \textit{Taylor series expansion} inspired by physics;
    \item Proposing an general \textit{self-supervised dynamics learning framework} that learns representations \textit{consistent among different temporal derivatives} with a \textit{balanced alternating learning strategy}, applicable to multiple existing self-supervised learning approaches;
    \item Demonstrating the \textit{data efficiency} and substantial \textit{performance gains} on common video representation learning tasks of the proposed method, and analyzing the learned dynamic features via \textit{attention and subspace clustering visualization}.
\end{itemize} 

==> sec/method.tex <==
\section{Approach}
\label{sec:approach}

In this section, we first describe the mathematical framework and explain our intuition through a thought experiment grounded in physics (\cref{sec:taylor}). Then describe in detail how we incorporate temporal differentiation with a balanced alternating learning strategy (\cref{sec:diff}) into two-stream self-supervised learning methods. We use SimCLR \cite{simclr} as a specific example for constructing and training a ViDiDi-based model while referring readers to other implementations in \cref{sec:objective}.


\subsection{Recover Hidden Views of Video Sequence}
\label{sec:taylor}

% \textcolor{red}{Change notations, so $C$ would consistently have one meaning}

\noindent \textbf{Taylor series expansion of videos.  }
We view one video not just as a sequence of $N$ discrete frames $[\bm{y}(n)]$, $n = 1, 2, \dots$, $N$, but as a continuous dynamic process $\bm{y}(t)$. We assume that this process is caused by latent factors, $\bm s$ and $\bm z$, which account for the static and dynamic aspects of the video through an unknown generative model:  
\begin{equation}
\bm y(t) = \bm g_{\bm 1}(\bm s) + \bm g_{\bm 2}(\bm z,t)
\label{eq:origin}
\end{equation}
where $\bm g_{\bm 1}(\bm s)$ generates a static environment and $\bm g_{\bm 2}(\bm z,t)$ generates a dynamic process situated in the environment. 

% \qq{In the following, maybe we can change $n$ to $t'$ and the deriative to should be with respect to $t'$}

Although $\bm y(t)$ is not observed, we can approximate $\bm y(t)$ for any time $t$ around specific time $n$ through the Taylor series expansion: 
\begin{equation}
\bm y(t) = \bm y(n) + (t-n) \frac{\partial \bm y}{\partial t}(n) + (t-n)^2\frac{1}{2!} \frac{\partial ^2 \bm y}{\partial t^2}(n) + \dots
\label{eq:taylor}
\end{equation}
Here, the original frame $\bm y(n)$ can be viewed as the zeroth order derivatives. Its contributions to $\bm y(t)$ do not incorporate a continuous time variable $t$. $\frac{\partial \bm y}{\partial t}(n) = \frac{\partial \bm g_{\bm 2}}{\partial t}(\bm z,n)$ and $\frac{\partial ^2 \bm y}{\partial t^2}(n) = \frac{\partial ^2 \bm g_{\bm 2}}{\partial t^2}(\bm z, n)$ are the first and second derivatives evaluated at time $n$, contributing to the underlying dynamics through linear and quadratic functions of time, respectively. 

The zeroth, first, or second derivatives provide different "views" of the continuous video dynamics. It is apparent that they share a common latent factor $\bm z$ but not $\bm s$, according to \cref{eq:origin}. Guiding the model to encode these views into consistent representations in the latent space provides a self-supervised learning strategy for reverse inference of the dynamic latent $\bm z$ rather than the static latent $\bm s$. Therefore, this strategy has the potential to better steer the model to uncover the hidden dynamics from discrete frames through temporal derivatives, which is often missed in traditional frame-based video learning and analysis.

\begin{figure}[t]
  \centering
   \includegraphics[width=.95\linewidth]{figure/graph_taylor2.pdf}
   \caption{\textbf{A thought experiment on physical motion.} The Taylor series expansion projects the dynamic process of a free fall motion onto three views expressed in terms of the height, velocity, and acceleration. The reverse inference of the common causes of the height, velocity, and acceleration leads to the encoding of the gravity $\bm g$ - the only variable pertaining to all three views, instead of unrelated static latents, $\bm {y_0}$ and $\bm {v_0}$.}
   \label{fig:taylor}
   % \vspace{-0.5cm}
   \vspace{-0.4cm}
\end{figure}

% \vspace{-0.3cm}
% \vspace{0.2cm}
\noindent \textbf{A thought experiment on physical motion.   }
Our idea is analogous to and inspired by physical motion. As illustrated in \cref{fig:taylor}, consider a 1-D toy example through a thought experiment . Imagine that we observe the free fall motion of a ball on different planets and aim to infer the planet based on a sequence of snapshots of the ball. The zeroth, first, and second derivatives are the position $\bm y(t)$, velocity $\bm v(t)$, and acceleration $\bm a(t)$, respectively. Evaluating these derivatives at discrete times $n$ gives rise to three sequences, providing different discrete views that collectively expand the continuous motion. Given the physical law, the free fall motion is governed by $\bm y(t) = \bm {y_0} + \bm {v_0}t-\frac{1}{2}\bm gt^2$, including three latent factors: the initial position $\bm {y_0}$, the initial velocity $\bm {v_0}$, and the gravity $\bm g$. It is straightforward to recognize that only the gravity $\bm g$ is involved in the position, velocity, and acceleration. Thus, inferring the representation shared across these different views reveals gravity $\bm g$, which is the defining feature of the dynamics.


\subsection{The ViDiDi Framework}
\label{sec:diff}
However, it is non-trivial to extend this intuition to practical learning of dynamics in natural videos. Next, we describe ViDiDi as a learning framework generalizable to multiple existing 2-stream self-supervised video representation methods. It involves 1) creating multiple views from videos through spatio-temporal augmentation and differentiating, 2) a balanced alternating learning strategy for pair-wise encoding of the different views into consistent representations, and 3) plugging this strategy into existing instance discrimination methods, including SimCLR \cite{simclr}, BYOL \cite{byol}, and VICReg \cite{vicreg}. See \cref{fig:general_method} for an overview. 

\begin{figure}[t]
\centering
  \includegraphics[width=0.9\textwidth]{figure/graph_method2.pdf}
  \caption{\textbf{Illustration of the ViDiDi framework.} For a batch of videos $\bm I$, we do two spatio-temporal augmentations $\bm \tau$ and $\bm \tau^{\prime}$ to obtain two batches of clips: $\bm V$ and $\bm V'$. These clips are evaluated for the $0^{th}$, $1^{st}$, or $2^{nd}$ order temporal derivatives. Such derivatives are further selected (denoted as $\bm X$ and $\bm X'$) via a balanced alternating learning strategy described in \cref{alg:schedule}. $\bm X$ and $\bm X'$ are the inputs to the video encoder in a 2-stream SSL framework such as SimCLR, BYOL, and VICReg for learning through instance discrimination. $\bm f$ is the video encoder, $\bm h$ is the MLP projection head, and $\bm Z$ and $\bm Z'$ are the encoded embeddings.}
  \label{fig:general_method}
  % \vspace{-0.5cm}
  \vspace{-0.3cm}
\end{figure}

% \vspace{0.1cm}
\noindent \textbf{Creating multiple views from videos.   }
i) \textit{\textbf{Augmentation}}: Given a batch of videos $\bm I$ in the shape of $\mathbb{R}^{B \times C \times L \times H \times W}$ where $B$ is the batch size, $L$ is the number of frames per video, $C$ is the number of channels, and $(H, W)$ is the frame size: we sample each video by randomly cropping two clips, each of length $T$. This is a temporal augmentation approach similar to previous works. For each clip, we apply a random set of spatial augmentations \cite{cvrl}, including random crops, horizontal flips, Gaussian blur, color jittering, and normalization. In this way, we create two augmented views for every video in the batch, denoted as $\bm V$ and $\bm V'$, each containing a batch of video clips in the shape of $\mathbb{R}^{B \times C \times T \times h \times w}$ where $(h, w)$ is the cropped frame size. See more details in the appendix. ii) \textit{\textbf{Differentiation}}: As introduced in \cref{sec:taylor}, we further recover hidden views of clips via temporal differentiation. For every augmented clip within either $\bm V$ or $\bm V'$, we evaluate its $0^{th}$, $1^{st}$, or $2^{nd}$ temporal derivatives. The clips in the same batch will be derived for the same number of times to better support learning of consistent representations across different order of derivatives. In this study, we limit the derivatives up to the $2^{nd}$ order which already shows significant improvements. Denote $\bm V(n) \in \mathbb{R}^{B \times C \times h \times w}$ as a batch of frames selected at time $n$ from the clip $\bm V$, we approximate temporal derivatives with finite forward differences, then the temporal derivatives with respect to $t$ and evaluated at $n$ are:
\vspace{-0.2cm}
\begin{align}
% \small
&\frac{\partial \bm V}{\partial t}(n) = \bm V(n+1) - \bm V(n) \\
&\frac{{\partial}^2 \bm V}{\partial t^2}(n) = \bm V(n+2) - 2*\bm V(n+1) + \bm V(n)
\end{align}
\vspace{-0.3cm}

% \vspace{-0.5cm}
% \vspace{0.1cm}
\noindent \textbf{Balanced alternating learning strategy.   }
We design a paring schedule for leaning consistent representations among derivatives and original frames for the same video using 2-stream SSL methods. Specifically, we define seven pairs: 
$(\bm V, \bm V')$, 
$(\bm V, \frac{\partial \bm V'}{\partial t})$, 
$(\frac{\partial \bm V}{\partial t}, \bm V')$, 
$(\frac{\partial \bm V}{\partial t}, \frac{\partial \bm V'}{\partial t})$, 
$(\frac{\partial \bm V}{\partial t}, \frac{\partial^2 \bm V'}{\partial t^2})$, 
$(\frac{\partial^2 \bm V}{\partial t^2}, \frac{\partial \bm V'}{\partial t})$, 
$(\frac{\partial^2 \bm V}{\partial t^2}, \frac{\partial^2 \bm V'}{\partial t^2})$, 
each including the temporal derivatives of $\bm V$ and $\bm V'$ evaluated for 0, 1, or 2 times. Such paired derivatives, denoted as $\bm X$ and $\bm X'$, provide inputs to two video encoders in separate streams. At each step (aka batch), we select one pair of derivatives following \cref{alg:schedule}. For each batch, the number of times $\bm V$ and $\bm V'$ each are derived in time, depends on the epoch number as well as additional randomness. Intuitively we choose this strategy to let learning of derivatives guide original frames in a balanced way. So we generally start by pairing the derivatives at higher orders, then the derivatives across different orders, and lastly the derivatives at the zeroth order, and continuing this cycle. We empirically verify that this balanced alternating learning strategy plays an important role in the learning process in the ablation study in \cref{sec:ablation}.

\RestyleAlgo{ruled}
\SetKwComment{Comment}{/* }{ */} 
\begin{algorithm}[ht]
\caption{Differentiation at Each \textbf{Batch}}
\label{alg:schedule}
\KwData{$\texttt{epoch} \geq 0$, ($\bm V$, $\bm V'$)}
\KwResult{($\bm X$, $\bm X'$)}
\tcp{Deterministic differentiation step}
\lIf{$\texttt{epoch} \texttt{\%} 4 = 0$}{
($\bm X$, $\bm X'$) $\gets$ ($\dfrac{\partial \bm V}{\partial t}$, $\dfrac{\partial \bm V'}{\partial t}$)
}
\lElseIf{$\texttt{epoch} \texttt{\%} 4 = 1$}{
($\bm X$, $\bm X'$) $\gets$ ($\dfrac{\partial \bm V}{\partial t}$, $\bm V'$)
}
\lElseIf{$\texttt{epoch} \texttt{\%} 4 = 2$}{
($\bm X$, $\bm X'$) $\gets$ ($\bm V$,$\dfrac{\partial \bm V'}{\partial t}$)
}
\lElse{
($\bm X$, $\bm X'$) $\gets$ ($\bm V$, $\bm V'$)
}
\tcp{Additional random differentiation step}
$\epsilon \gets \texttt{rand}(0,1)$\;
\lIf{$\epsilon < 0.5$}{
($\bm X$, $\bm X'$) $\gets$ ($\dfrac{\partial \bm X}{\partial t}$, $\dfrac{\partial \bm X'}{\partial t}$)
}
\end{algorithm}

\noindent \textbf{Plug into existing instance discrimination methods. } Our approach is generalizable to different types of instance discrimination methods, including SimCLR \cite{simclr} based on contrastive learning, BYOL \cite{byol} using teacher-student distillation, and VICReg \cite{vicreg} via variance-invariance-covariance regularization. The above methods are selected as representative examples. By integrating ViDiDi with these different learning objectives, we have trained and tested various models, namely, ViDiDi-SimCLR, ViDiDi-BYOL, and ViDiDi-VIC. We describe ViDiDi-SimCLR below and refer to the appendix for details about other models. $(\bm X, \bm X')$ are two batches of input to the two streams of video encoders, denoted as $f$, which uses a 3D ResNet or other architectures in our experiments. Following the video encoder, $h$ is a multi-layer perceptron (MLP) based projection head, yielding paired embeddings $(\bm Z, \bm Z')$, $Z=\left[z_1, \ldots, z_B\right]^{T} \in \mathbb{R}^{B \times D}$. We evaluate the representational similarity between the $i^{th}$ clip and the $j^{th}$ clip as $s_{i, j}=\bm{z}_i^{\top} \bm{z}'_j /\left(\left\|\bm{z}_i\right\|\left\|\bm{z}'_j\right\|\right)$. Given a batch size of $B$, the InfoNCE loss \cite{simclr} is:
\begin{equation}
% \small
    \mathcal{L}_{NCE}
    =
    \frac{1}{2B}\sum_{i=1}^B
    \log \frac{\exp ( s_{i, i}/ \alpha )}{\sum_{j=1}^B \exp (s_{i, j} / \alpha)}
    +
    \frac{1}{2B}\sum_{i=1}^B
    \log \frac{\exp ( s_{i, i}/ \alpha) }{\sum_{j=1}^B \exp (s_{j, i} / \alpha)}
\end{equation}



==> sec/related_works.tex <==
\section{Relationship to Prior Arts}
\label{sec:relatedwork}

% \syc{Shrink}

% \textcolor{red}{Discuss relationship and differences from previous works category by category, and emphasize discussion with optical flow.}

Current methods for SSL of video representations mainly utilize instance discrimination, pretext tasks, multimodal learning, and other ones. In the following, we discuss these results, and highlight the advantages of our method over existing ones.

\noindent \textbf{Instance discrimination.   } 
It is first applied to images \cite{simclr, byol, moco, swav} and then to videos \cite{videomoco, rbyol, cvrl, cacl, vthcl, coclr, tequi}. Given either images or videos as instances, models learn to discriminate different instances versus different "views" of the same instance, where the views are generated by spatio-temporal augmentations \cite{videomoco, cvrl}. The learning process is driven by contrastive learning \cite{cvrl}, clustering \cite{videomoco}, or teacher-student distillation \cite{rbyol}. Recognizing the rich dynamics in videos, some prior works have further modified the loss function to consider each video's temporal attributes, such as play speed \cite{vthcl}, time differences \cite{cvrl, ltn, tclr, rbyol}, frame order \cite{dsm}, and motion diversity \cite{tclr, fima}. Such modifications do not fully capture the essence of videos as reflections of continuous real-world dynamics, and are usually designed for a specific instance discrimination method. Apart from being applicable to different frameworks of instance discrimination, our approach, is new for its extraction of continuous dynamics by unfolding a video's hidden views via Taylor expansion and temporal differentiation.

\noindent \textbf{Pretext tasks.   } Another category of methods involves creating learning tasks from videos. These tasks have many possible variations, such as identifying transformations applied to videos \cite{rtt, 3drotnet}, predicting the speed of videos \cite{speednet, rspnet, pacepred, prp, vpsp}, identifying incorrect ordering of frames or clips \cite{shufflelearn, o3n, voss, dave2023shortcuts}, resorting them in order \cite{opn, vcop}, and solving space-time puzzles \cite{3dstpuzzle, videojigsaw}. The above methods usually require a complex combination of different tasks to learn general representations, while some recent works utilize large transformer backbones and learn by reconstructing masked areas \cite{tong2022videomae} and further incorporating motion guidance into masking or reconstruction \cite{maskmotion, motionguide}. These tasks provide non-trivial challenges for models to learn but are unlikely to reflect the natural processes through which humans and machines alike may learn and interpret dynamic visual information. In contrast, ViDiDi uses simple learning objectives and models how the physical world can be intuitively processed and understood without the need for complex tasks.

\noindent \textbf{Others.   } 
In addition, prior methods also learn to align videos with other modalities, such as audio tracks \cite{fac, brave, avts}, video captions \cite{fac, cpd, milnce, emcl}, and optical flows \cite{coclr, brave, Li2021MotionFocusedCL, Ni2022MotionSC, CRAFT}. Optical flow also models changes between frames and is related to our method. However, our method is easy to calculate and intuitively generalize to higher orders of motion and guides the learning of the original frames within the same encoder in contrast to an additional encoder for optical flow \cite{coclr}. Besides, our temporal differentiation strategy may be flexibly adapted to other dynamic data such as audio while optical flow explicitly models the movements of pixels. Incidentally, our proposed \textit{balanced alternating learning strategy} as a simple yet novel way of learning different types of data, may inspire multimodal learning. Some other existing works manipulate frequency content to create augmented views of images \cite{FAMLPAF, Xu2021AFF, xray} or videos \cite{freqaug, MitigatingAE, Li2021MotionFocusedCL} to make models more robust to out-of-domain data. Related to but unlike these works, we seek a fundamental and computationally efficient strategy to construct views from videos that reflect the continuous nature of real-world dynamics. Besides, apart from a new way of processing data, we propose an alternating learning strategy that is pivotal to boosting learning and has not been explored in previous works.

==> sec_arxiv/checklist.tex <==
\clearpage

\section*{NeurIPS Paper Checklist}

% %%% BEGIN INSTRUCTIONS %%%
% The checklist is designed to encourage best practices for responsible machine learning research, addressing issues of reproducibility, transparency, research ethics, and societal impact. Do not remove the checklist: {\bf The papers not including the checklist will be desk rejected.} The checklist should follow the references and follow the (optional) supplemental material.  The checklist does NOT count towards the page
% limit. 

% Please read the checklist guidelines carefully for information on how to answer these questions. For each question in the checklist:
% \begin{itemize}
%     \item You should answer \answerYes{}, \answerNo{}, or \answerNA{}.
%     \item \answerNA{} means either that the question is Not Applicable for that particular paper or the relevant information is Not Available.
%     \item Please provide a short (1–2 sentence) justification right after your answer (even for NA). 
%    % \item {\bf The papers not including the checklist will be desk rejected.}
% \end{itemize}

% {\bf The checklist answers are an integral part of your paper submission.} They are visible to the reviewers, area chairs, senior area chairs, and ethics reviewers. You will be asked to also include it (after eventual revisions) with the final version of your paper, and its final version will be published with the paper.

% The reviewers of your paper will be asked to use the checklist as one of the factors in their evaluation. While "\answerYes{}" is generally preferable to "\answerNo{}", it is perfectly acceptable to answer "\answerNo{}" provided a proper justification is given (e.g., "error bars are not reported because it would be too computationally expensive" or "we were unable to find the license for the dataset we used"). In general, answering "\answerNo{}" or "\answerNA{}" is not grounds for rejection. While the questions are phrased in a binary way, we acknowledge that the true answer is often more nuanced, so please just use your best judgment and write a justification to elaborate. All supporting evidence can appear either in the main paper or the supplemental material, provided in appendix. If you answer \answerYes{} to a question, in the justification please point to the section(s) where related material for the question can be found.

% IMPORTANT, please:
% \begin{itemize}
%     \item {\bf Delete this instruction block, but keep the section heading ``NeurIPS paper checklist"},
%     \item  {\bf Keep the checklist subsection headings, questions/answers and guidelines below.}
%     \item {\bf Do not modify the questions and only use the provided macros for your answers}.
% \end{itemize} 
 

%%% END INSTRUCTIONS %%%


\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The abstract introduced the paper's contributions and scope in proposing a new self-supervised video dynamics learning method presented in \Cref{sec:approach} and \Cref{sec:experiments}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A No or NA answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We provide discussions on limitations and future directions in \Cref{sec:discussion}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper has no limitation while the answer No means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate "Limitations" section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory Assumptions and Proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We do not propose theorems in the paper.  
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

    \item {\bf Experimental Result Reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We clearly explained the proposed methods and algorithms in \Cref{sec:approach}, as well as experiment setup in \Cref{sec:experiments} and \Cref{sec:detail}. The code will be released upon acceptance.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item If the paper includes experiments, a No answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and/or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerNo{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We haven't provided an open access code with detailed instructions upon submission, but will provide an open access code with detailed instructions upon acceptance.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so “No” is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental Setting/Details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer, etc.) necessary to understand the results?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We clearly explained the proposed methods and algorithms in \Cref{sec:approach}, as well as experiment setup in \Cref{sec:experiments} and \Cref{sec:detail}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment Statistical Significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We conduct main experiments for at least 3 times. We follow the standard train/val/test splits of the datasets.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The authors should answer "Yes" if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g. negative error rates).
        \item If error bars are reported in tables or plots, The authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments Compute Resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: The required computing resources are justified in \Cref{sec:detail}.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code Of Ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We follow the NeurIPS Code of Ethics.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer No, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader Impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We discuss the potential inspiration of the work to both machine vision and neuroscience.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that there is no societal impact of the work performed.
        \item If the authors answer NA or No, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pretrained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: Our paper does not have such risks.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We properly cited and credited existing models and datasets.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New Assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerYes{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We describe the proposed new frameworks and algorithms in details.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset/code/model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and Research with Human Subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We do not involve human subjects.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional Review Board (IRB) Approvals or Equivalent for Research with Human Subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: We do not involve human subjects.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\end{enumerate}
